15000 Ellipsoidal Binary Candidates in TESS: Orbital Periods, Binary Fraction, and Tertiary Companions

We present a homogeneously-selected sample of 15779 candidate binary systems with main sequence primary stars and orbital periods shorter than 5 days. The targets were selected from TESS full-frame image lightcurves on the basis of their tidally-induced ellipsoidal modulation. Spectroscopic follow-up suggests a sample purity of $83 \pm 13$ per cent. Injection-recovery tests allow us to estimate our overall completeness as $28 \pm 3$ per cent with $P_\mathrm{orb} < 3$ days and to quantify our selection effects. We estimate that $39 \pm 4$ per cent of our sample are contact binary systems, and we disentangle the period distributions of the contact and detached binaries. We derive the orbital period distribution of the main sequence binary population at short orbital periods, finding a distribution continuous with the log-normal distribution previously found for solar-type stars at longer periods, but with a significant steepening at $P_\mathrm{orb} \lesssim 3$ days, and a pile-up of contact binaries at $P_\mathrm{orb} \approx 0.4$ days. Companions in the period range 1--5 days are found to be an order of magnitude more frequent around stars hotter than $\approx 6250 K$ (the Kraft break) when compared to cooler stars, suggesting that magnetic braking plays an important role in shaping the temperature and period distributions. We detect resolved tertiary companions to $9.0 \pm 0.2$ per cent of our binaries with a median separation of 3200 AU. The frequency of tertiary companions rises to $29 \pm 5$ per cent among the systems with the shortest ellipsoidal periods. This large binary sample with quantified selection effects will be a powerful resource for future studies of detached and contact binary systems with $P_\mathrm{orb} < 5$ days.

==> mass_ratios.tex <==






\subsection{Mass Ratio}
\label{sec:mass-ratio}


\begin{figure*}
\includegraphics[width=\columnwidth]{figures/violin_plot_tell_period.pdf}
\includegraphics[width=\columnwidth]{figures/violin_plot_simulation.pdf}
\includegraphics[width=\columnwidth]{figures/violin_plot_tell_mass.pdf}
\includegraphics[width=\columnwidth]{figures/violin_plot_simulation_mass.pdf}
\caption{\cmnt{TBD. Change variable name}
}
\label{fig:mass-ratio-violins}
\end{figure*}

\begin{figure}
\includegraphics[width=\columnwidth]{figures/tell_histogram.pdf}
\caption{\cmnt{TBD}
}
\label{fig:mass-ratio-distribution}
\end{figure}

In principle, it is possible to estimate the mass ratio of a BEER binary on the basis of its measured ellipsoidal and Doppler beaming amplitudes, using the equations detailed in Section~\ref{sec:beer}.
However, in practise, the measured amplitude of the Doppler beaming may not be as secure as the ellipsoidal and reflection amplitudes.
Due to the comparatively small amplitude of the beaming signal, it is significantly more vulnerable to being measured incorrectly as a result of other small-scale variability from the system.
We therefore prefer to focus our analysis on the ellipsoidal amplitude alone.

Using just the ellipsoidal amplitude, it is not possible to estimate the mass ratio for an individual target. 
It is only possible to measure a function that we name the `ellipsoidal mass function', which can be found by rearranging Equation~\ref{eq:ell2}:
\begin{align}
\label{eq:yell}
\mathcal{Y} &= - \frac{a_\text{2c}}{\text{1\,ppm}} \frac{M_1}{M_\odot} \left(\frac{R_1}{R_\odot}\right)^{-3} \left(\frac{P}{\text{1\,day}}\right)^2 \frac{1}{13400 \alpha_\text{e2,2}}\\
 &= \frac{q}{q+1} \sin^2 i 
\end{align}
where $q = M_2 / M_1$ is the mass ratio of the binary. An assumption has been here that the primary star dominates the flux of the binary, such that $f_1 / f_2 >> 1$ in Equation~\ref{eq:ell2}.

Using an assumed distribution of the orbital inclination $i$, it is possible to disentangle the distribution of $q$ from that of $i$ in the aggregate. 
We emphasise that this is not a method to estimate $q$ for any individual binary system, but a method to estimate the overall distribution of $q$ across the sample.
The methodology is detailed by \citet{Shahaf2021}, who show that the cumulative distribution function of $\mathcal{Y}$ behaves, in aggregate across the sample, in a similar way to $q$. It can be calculated by
\begin{equation}
\label{eq:tell}
\mathcal{T} = 1 - \sqrt{1 - 2 \mathcal{Y}} + \frac{\mathcal{Y}}{2\sqrt{1-\mathcal{Y}}} \ln \left(\frac{\sqrt{1-\mathcal{Y}} + \sqrt{1 - 2 \mathcal{Y}}}{\sqrt{1 - \mathcal{Y}} - \sqrt{1 - 2 \mathcal{Y}}} \right)
\end{equation}


A number of caveats should be born in mind. 
Firstly, in deriving Equation~\ref{eq:yell}, a simplifying assumption was made that the secondary star's flux contribution is negligible.
For binaries with $q<<1$ such an assumption is valid, and for binaries with $q \approx 1$ the predicted ellipsoidal amplitude should not be affected by this assumption\footnote{In the twin-mass case, both stars will have a the same flux contribution and the same ellipsoidal amplitude, so neglecting one star's light will have no effect on the overall amplitude.}. 
For $q$ values in the middle of the range, this assumption may cause $q$ to be under-estimated by of order a few tens per cent of its true value.
Secondly, in deriving Equation~\ref{eq:tell}, an assumption is made by \citep{Shahaf2021} that the distribution of $\cos i$ is uniform. 
In our sample this is not the case, given the selection effects on $i$ shown in Figure~\ref{fig:cornerplot}.
In the following analysis we will always compare the distribution of \tell\ derived from our sample with one derived from a simulated sample that has been passed through the same selection process and has been analysed in the same way
As a result, any biases that may be introduced by the issues discussed here should equally affect both the real and simulated samples.





\citet{Moe2017} measured mass ratio distributions from several samples of binaries across a range of stellar types and orbital periods. 
The most similar to our sample in terms of orbital period is a sample of 32 double-lined spectroscopic binaries \citep{sources?} with periods of 2--20\,days and O and early-B stellar types.
From this sample, they measure $\gamma_\mathrm{large} = -0.3 \pm 0.3$ and a twin fraction $F_\mathrm{twin} = 0.11 \pm 0.04$ (their Fig.~8). 
In terms of stellar type, our sample is dominated by AFGK stars.
\citet{Moe2017} analyze one sample with stellar types B6--A7, which includes 36 binaries with orbital periods in the range 20--80\,000 days and $0.15 < q < 0.75$ \citep[sample from][]{Gullikson2016}.
They measure $\gamma_\mathrm{small} = 0.7 \pm 0.8$ and $\gamma_\mathrm{large} = -1.0 \pm 0.5$. 
FGK stars:
flogp, q > 0.3 = 0.017 pm 0.007
gamma small = 0.3 pm 0.9
gamma large = -0.6 pm 0.7
ftwin = 0.29 pm 0.11
And then the big table 13 is interpolated from individual studies



\begin{table*}
\caption{?????}
\begin{tabular}{lcccccccc}
\label{tab:other-surveys}
Sample & Period [days] & Stellar Type & Sample Size & $f_{\log P}$ & $q_\mathrm{break}$ & $\gamma_\mathrm{small}$ & $\gamma_\mathrm{large}$ & $F_\mathrm{twin}$ \\
\hline
\textit{Moe-SB2} & 2--20 & OB & 32 & Various & $0.3$ & -- & $-0.3 \pm 0.3$ & $0.11 \pm 0.04$ \\
\textit{Moe-Gullikson} & 20--80k & BA & 36 & $0.06 \pm 0.02$ & $0.3$ & $0.7 \pm 0.8$ & $-1.0 \pm 0.5$ & -- \\
\textit{Moe-Raghavan} & <100 & FGK & 14 & $0.015 \pm 0.007$ & $0.3$ & $0.3 \pm 0.9$ & $-0.6 \pm 0.7$ & $0.29 \pm 0.11$ \\
\textit{Moe-Interpol-AB} & 10 & BA & -- & $0.07 \pm 0.02$ & $0.3$ & $0.2 \pm 0.4$ & $-0.5 \pm 0.3$ & $0.22 \pm 0.07$ \\
\textit{Moe-Interpol-FGK} & 10 & FGK & -- & $0.027 \pm 0.009$ & $0.3$ & $0.3 \pm 0.4$ & $-0.5 \pm 0.3$ & $0.30 \pm 0.09$ \\
\textit{ElBadry-AF} & 60k--1.2M & AF & ?? & -- & $0.3$ & $0.1 \pm 1.0$ & $-0.9 \pm 1.0$ & $0.09 \pm 0.07$ \\
\textit{ElBadry-FGK} & 100k--1.7M & FGK & ?? & --& $0.5$ & $0.1 \pm 0.7$ & $-1.2 \pm 0.7$ & $0.10 \pm 0.03$ \\
\textit{This work $(P > 1)$} & 1--5 & AFG & ?? & $0.01213(7)$ & $0.40 \pm 0.02$ & $0.6 \pm 0.1$ & $-1.2 \pm 0.1$ & $0.000 \pm 0.001$ \\

\end{tabular}
\end{table*}




